Learning to Learn Financial Networks for Optimising Momentum Strategies

Network momentum provides a novel type of risk premium, which exploits the interconnections among assets in a financial network to predict future returns. However, the current process of constructing financial networks relies heavily on expensive databases and financial expertise, limiting accessibility for small-sized and academic institutions. Furthermore, the traditional approach treats network construction and portfolio optimisation as separate tasks, potentially hindering optimal portfolio performance. To address these challenges, we propose L2GMOM, an end-to-end machine learning framework that simultaneously learns financial networks and optimises trading signals for network momentum strategies. The model of L2GMOM is a neural network with a highly interpretable forward propagation architecture, which is derived from algorithm unrolling. The L2GMOM is flexible and can be trained with diverse loss functions for portfolio performance, e.g. the negative Sharpe ratio. Backtesting on 64 continuous future contracts demonstrates a significant improvement in portfolio profitability and risk control, with a Sharpe ratio of 1.74 across a 20-year period.

==> backtest-v20230709/perf_table_raw.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Raw Signals}
\label{tab:bt_perf_table_raw}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &   ret &   vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.036 & 0.053 &   0.671 &               0.037 &         0.200 &                 17.2\% &    0.951 &   0.173 &    53.9\% &                 0.955 \\
MACD      & 0.025 & 0.047 &   0.533 &               0.033 &         0.121 &                 27.5\% &    0.766 &   0.200 &    52.9\% &                 0.977 \\
LinReg    & 0.043 & 0.042 &   1.029 &               0.028 &         0.080 &                 11.5\% &    1.541 &   0.538 &    53.6\% &                 1.031 \\
GLinReg   & 0.060 & 0.049 &   1.227 &               0.033 &         0.085 &                  7.7\% &    1.806 &   0.713 &    54.3\% &                 1.034 \\
L2GMOM    & 0.065 & 0.047 &   1.400 &               0.030 &         0.066 &                  7.2\% &    2.197 &   0.942 &    50.7\% &                 1.086 \\
L2GMOM\_SR & 0.045 & 0.032 &   1.394 &               0.023 &         0.052 &                  6.2\% &    1.911 &   0.817 &    52.0\% &                 1.051 \\
\bottomrule
\end{tabular}
\end{table}


==> backtest-v20230709/perf_table_scaled.tex <==
\begin{table}
\centering
\caption{Performance Metrics - Rescaed to 15% Target Volatility}
\label{tab:bt_perf_table_scaled}
\begin{tabular}{lrrrrrrrrrr}
\toprule
{} &   ret &   vol &  sharpe &  downside deviation &  max drawdown & max drawdown duration &  sortino &  calmar & hit rate &  avg profit over loss \\
\midrule
Long Only & 0.117 & 0.148 &   0.792 &               0.095 &         0.633 &                 17.1\% &    1.229 &   0.177 &    53.9\% &                 0.969 \\
MACD      & 0.102 & 0.147 &   0.694 &               0.094 &         0.342 &                 23.7\% &    1.085 &   0.279 &    52.9\% &                 0.997 \\
LinReg    & 0.174 & 0.147 &   1.189 &               0.092 &         0.285 &                 11.9\% &    1.892 &   0.623 &    53.6\% &                 1.049 \\
GLinReg   & 0.200 & 0.147 &   1.365 &               0.093 &         0.253 &                  8.9\% &    2.149 &   0.822 &    54.3\% &                 1.048 \\
L2GMOM    & 0.224 & 0.147 &   1.525 &               0.089 &         0.186 &                  7.2\% &    2.531 &   1.201 &    50.7\% &                 1.099 \\
L2GMOM\_SR & 0.255 & 0.146 &   1.744 &               0.094 &         0.173 &                  5.7\% &    2.716 &   1.495 &    52.0\% &                 1.091 \\
\bottomrule
\end{tabular}
\end{table}


==> bin/4-Backtest-v20230627.tex <==
\section{Performance Evaluation}
% backtest-v20230709
% - (1) adding GraphLinReg (alpha = 0.05)

\label{sec:backtest}

\subsection{Backtest Setup}
\subsubsection{Dataset}
The backtest was implemented using 64 ratio-adjusted continuous future contracts from the Pinnacle Data Crop CLC Database. These contracts mainly contain four classes of assets, that is, Commodities, Equities, Fixed Income and Currencies. The daily price data are available from 1990 to 2022, although different assets could have different time spans when the prices are available. In Appendix, Table \ref{table:universe} lists all the assets in backtest. 

\subsubsection{Momentum Features}  \label{sec:subsec:momentum_features}
The following eight features were included:
\begin{itemize}
    \item{\textbf{Volatility normalised returns}} over the past 1-day, 1-month, 3-month, 6-month and 1-year periods; defined as $\rfrac{r_{t-\Delta:t}}{\sigma_t \sqrt{\Delta}}$, where $\sigma_t$ is an ex-ante daily volatility estimated from an exponential weighted moving standard deviation with 60-day span on daily return. 
    \item{\textbf{MACD} indicators} with three combinations of short and long time scales $(S_k, L_k) \in \{(8,24), (16, 48), (32, 96)\}$.
\end{itemize}
We further adopted a data winsorisation strategy in order to mitigate the influence of outliers. Specifically, each feature of each asset was capped and floored to fall within a range defined by five times its exponentially weighted moving standard deviations from its corresponding exponentially weighted moving average. This computation was carried out using a half-life of 252 days. 

\subsubsection{Graph Learning Details} 
The first step is to decide the feature matrix $\mathbf{V}$ as the input of graph learning module. We chose the same momentum features in Section \ref{sec:subsec:momentum_features} as $\mathbf{V}$. At each day, we look back $\delta$ days, where the node set of a graph is defined as the union of assets that have less than 10\% missing values in this $\delta$-day window of momentum features. Since different assets have different time periods when the prices are available, graphs could have different sizes. In generating network momentum features with proposed GMOM and L2GMOM, we combined $K = 5$ different graphs learned from  five different lookback windows such that $\delta \in \{252, 504, 756, 1008, 1260\}$.

\subsubsection{Strategy Candidates}
For comparison against traditional time-series momentum strategies, we compare the proposed strategies against the following reference benchmarks:
\begin{itemize}
    \item{\textbf{Long Only}} takes a consistent long position $x_{i,t} = 1$ with daily volatility scaling. 
    \item{\textbf{MACD}} [ref eq]
    \item{\textbf{LinReg}} stands for Linear Regression with the eight \textit{momentum features} as input, and the [ref eq] as target. 
\end{itemize}
We name the strategies constructed from the proposed models as \textbf{GMOM} in Eq.\eqref{eq: gmom}, \textbf{GMOM\_SR} in Eq.\eqref{eq: gmom_sr}, \textbf{L2GMOM} in Eq.\eqref{eq:l2gmom} and  \textbf{L2GMOM\_SR} in Eq.\eqref{eq:l2gmom_sr}.

\subsubsection{Optimisation Details} 
The models were trained every 5 years. This process involved coefficient optimisation and hyperparameter tuning using all preprocessed data up to the point of re-calibration. Afterwards, these optimised models were used to generate trading signals for the subsequent 5 years, using out-of-sample data. To ensure an adequate number of training samples, the first backtest period comprised of 1990-1999 for training, followed by 2000-2004 for testing. Likewise, the second period included 1990-2004 for training, and then 2005-2009 for testing. Therefore, we have an aggregated 20-year out-of-sample period from 2000 to 2020. For each backtest period, the most recent 10\% of training data was set aside as a validation set for hyperparameter tuning.

For linear models like LinReg and GMOM, there are analytical solutions. For L2GMOM, GMOM\_SR, and L2GMOM\_SR, we employed stochastic gradient descent using the \texttt{Adam} optimiser in a mini-batch approach. The validation set was utilised to determine convergence, activating early stopping when the moving average validation loss failed to improve beyond a certain threshold. To reduce the randomness introduced by the \texttt{Adam} optimiser, we carried out the experiments over 5 runs with random initial values and averaged the model outputs to create an ensemble.

\subsection{Portfolio Performance}

%\input{backtest-v20230627/perf_table_raw}
%\input{backtest-v20230627/perf_table_scaled}
\input{backtest-v20230627/perf_table_combine}

In evaluating the portfolio performance, we use the following annualised metrics in Table \ref{tab:bt_perf_table_raw}:
\begin{itemize}
    \item{\textbf{Profitability Measures}}: expected return and hit rate (the percentage of days with positive returns across the test period)
    \item{\textbf{Risk Measures}}: daily volatility (vol.), downside deviation, maximum drawdown (MDD) and MDD duration (the percentage of days with MDD across the test period).
    \item{\textbf{Overall Performance Measures}}: Sharpe ratio (expected return$/$vol.), Sortino ratio (expected return$/$downside deviation), Calmar ratio (expected return$/$MDD), and the average profits over the average loss ($\frac{\text{Avg. P}}{\text{Avg. L}}$).
\end{itemize}%

In order to have a better comparison between different strategies, we apply an additional layer of volatility scaling at the portfolio level to an annualised volatility target of 15\% and report the above evaluation metrics in Table \ref{tab:bt_perf_table_scaled}. 

In Figure \ref{subfig:cumulative_returns_raw} and Figure \ref{subfig:cumulative_returns_scaled}, we plot the daily cumulative returns of raw signals and signals scaled to 15\% annual volatility of main strategies. 
% [whether we should include the SR curves here?]

% describe the table. 
% descebe the Figures. 


\begin{figure*}[h]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_pnl_raw.png}
        \caption{Raw signals}
        \label{subfig:cumulative_returns_raw}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_pnl_scaled.png}
        \caption{Signals scaled to 15\% volatility target}
        \label{subfig:cumulative_returns_scaled}
    \end{subfigure}
\caption{Cumulative Returns}
\label{fig:cumulative_returns}
\end{figure*}


\subsection{Orthogonal Analysis}

To evaluate whether the signals constructed from the proposed models are different from the reference baselines, we calculated the \textit{correlation} of daily returns between candidate signals in Figure \ref{subfig:bt_corr}. Besides, we calculate the percentage by how much the daily signals of two strategies have the same direction, also known as \textit{sign agreement} in Figure \ref{subfig:sign_agreemtn}. 


\begin{figure*}[h!]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/bt_corr_scaled.png}
        \caption{Return Correlations - Scaled to 15\% Volatility Target}
        \label{subfig:bt_corr}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/sign_agreement.png}
        \caption{Sign Agreement}
        \label{subfig:sign_agreemtn}
    \end{subfigure}
\caption{Orthogonal Analysis: Correlations and Sign Agreement}
\label{fig:cumulative_returns}
\end{figure*}


\subsection{Turnover Analysis}

Whether the signals make money after considering the turnover


\begin{figure*}[h!]
    \centering
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/avg_turnover.png}
        \caption{Average Turnover}
        \label{subfig:corr}
    \end{subfigure}
    \hspace{0.1cm}
    \begin{subfigure}[]{0.49\textwidth}
        \includegraphics[width=1\textwidth]{backtest-v20230627/sr_turnover.png}
        \caption{Sharpe Ratio under different cost}
        \label{subfig:sign_agreemtn}
    \end{subfigure}
\caption{Turnover Analysis}
\label{fig:cumulative_returns}
\end{figure*}




\subsection{Momentum Spillover Analysis}

% we plot certain graphs that we obtained here to explain the performance gain.

% more literature.

\subsection{Momentum or Mean Revision}

In GMOM and L2GMOM, we restrict the graph adjacency matrix only with non-negative entries whose value reflect the momentum spillover effects between two assets. So the graph momentum features reflect the momentum trends of target assets. However, since we applied linear model whether the coefficients are learned. Therefore, negative coefficients may contradict the basic philosophy of momentum strategy. 

In figure , we plot the change of graph momentum/momentum coefficients. 

literature?



==> bin/proposal.tex <==

The weighted graph adjacency matrix $\mathbf{A}_t$ is expected to reflect the strength of how similar these assets are in the feature space. The entries of $\mathbf{A}_t$ should be non-negative, so the momentum feature from different peer assets are not cancelled out in Eq.\eqref{eq: network_momentum}. Here, we consider the following graph learning model \cite{kalofoliasHowLearnGraph2016}:
\begin{equation}
\label{eq: gl}
\begin{aligned}
    \min_{\mathbf{A}_t} & ~~  \text{tr}\Big(\mathbf{V}_t^{\top}(\mathbf{D}_t -\mathbf{A}_t) \mathbf{V}_t \Big)- \alpha \mathbf{1}^{\top} \log (\mathbf{A}_t \mathbf{1})+ \beta ||\mathbf{A}_t||_F^2  \\
    s.t. & ~~  \mathbf{A}_{ij, t} = \mathbf{A}_{ji, t}, ~~ \mathbf{A}_{ij, t} \geq 0 ~~ \forall i \neq j
\end{aligned}
\end{equation}%
where $\mathbf{D}_t$ is a diagonal matrix with $\mathbf{D}_{ii,t} = \sum_j \mathbf{A}_{ij,t}$. \par

% why we use the above model?
The first trace term in Eq.\eqref{eq: gl} is derived from spectral smoothness with a mild assumption that momentum features are low-pass graph signal, which is consistent with the finding that multi-asset financial time series are a low-pass graph signal that exhibits communities \cite{ramakrishnaUserGuideLowPass2020}. Note that, the trace term is linear in the dot product of any pair of momentum features. \par  

The second term is a log regularisation on node degree, which is added to avoid any assets without any connection. There are two hyperparameters $\alpha$ and $\beta$. Together they control the topological properties of learned graph, such as sparsity. The choice of $\alpha$ and $\beta$ can largely affect the performance of portfolio.  \par

The optimisation in Eq.\eqref{eq: gl} is convex and hence can be solved with a guarantee of global minimum. 
